Zero-shot User Intent Detection via Capsule Neural Networks

User intent detection plays a critical role in question-answering and dialog systems. Most previous works treat intent detection as a classification problem where utterances are labeled with predefined intents. However, it is labor-intensive and time-consuming to label users' utterances as intents are diversely expressed and novel intents will continually be involved. Instead, we study the zero-shot intent detection problem, which aims to detect emerging user intents where no labeled utterances are currently available. We propose two capsule-based architectures: INTENT-CAPSNET that extracts semantic features from utterances and aggregates them to discriminate existing intents, and INTENTCAPSNET-ZSL which gives INTENTCAPSNET the zero-shot learning ability to discriminate emerging intents via knowledge transfer from existing intents. Experiments on two real-world datasets show that our model not only can better discriminate diversely expressed existing intents, but is also able to discriminate emerging intents when no labeled utterances are available.

==> dataset.tex <==
\begin{table}[h!]
\centering
\resizebox{8cm}{!}{% <-
\begin{tabular}{l|l|l}
\hline
\textbf{Dataset} & \textbf{SNIPS-NLU} & \textbf{CVA} \\\hline   
Vocab Size   &  10,896 & 1,709\\
Number of Samples   &  13,802    &  9,992  \\
Average Sentence Length   &  9.05    & 4\\
Number of Existing Intents   &  5   & 80\\
Number of Emerging Intents  &  2   & 20\\\hline
\end{tabular}
}
\vspace{0.1in}
\caption{Dataset statistics.}
\label{data_statistics}
\end{table}
